Instabilities, nucleation, and critical behavior in nonequilibrium driven fluids: theory and simulation

The main subject of this thesis rests on the study ---at different levels of description--- of instabilities in systems which are driven, i.e., maintained far from equilibrium by an external forcing. We focus here on two main classes, namely, driven--diffusive fluids and driven granular gases. A particular driven-diffusive lattice model, prototype for nonequilibrium phase transitions, is investigated. A well-known disadvantage of lattice models is that, when they are compared directly with experiment, often do not account for important features of the corresponding nonequilibrium phase diagram, such as structural, morphological, and even critical properties. Furthermore, theoreticians often tend to consider them as prototypical models for certain behavior, a fact which is in many cases not justified. This is discussed in the first part of this thesis, where we introduce a novel, realistic model for computer simulation of anisotropic fluids. The second class of systems we consider in this thesis concerns driven granular gases. We study clustering, symmetry breaking, and phase separation instabilities in two-dimensional driven granular gases, using both molecular dynamics simulations and granular hydrodynamics. Hydrostatic predictions are tested by comparing with molecular dynamics simulations. We are able to develop an effective Langevin description for close-packed macroparticle, confined by a harmonic potential and driven by a delta-correlated noise.

==> agradec.tex <==
\chapter{Acknowledgments}
Esta etapa de mi vida se cierra con dos nacimientos: en marzo, mi hija Cora y ahora, esta tesis. Mientras que las sensaciones que me produce el primero quedan en familia, debo expresar aqu\'i mi agradecimiento a quienes han contribuido al segundo.

En primer lugar quiero agradecer a Joaqu\'in Marro, mi profesor, tutor y mentor, todo el apoyo incondicional que me ofreci\'o desde el principio, sabiendo siempre qu\'e era lo mejor para m\'i en cada momento. A Pedro Garrido le agradezco todo el tiempo dedicado, su modo tan especial de motivar, las muchas dudas resueltas y las planteadas tambi\'en, y su franqueza. Parte de este trabajo se la debo a la intuici\'on de Paco de los Santos, mi compa\~nero de despacho con el que he compartido muy buenos ratos y charlas sinceras y de cuyo humor inteligente he disfrutado. Asimismo agradezco a Miguel \'Angel Mu\~noz, para m\'i un modelo a seguir, su inter\'es, apoyo y consejo en momentos muy oportunos. Y al resto de los componentes del grupo de F\'isica Estad\'istica: Omar, mi compa\~nero de viaje durante estos \'ultimos cuatro a\~nos, siempre cordial, altruista y dispuesto, David Navidad, Jes\'us Cort\'es, Pablo Hurtado, Abdelfattah Achahbar, Antonio L. Lacomba, Joaqu\'in Torres, Don Jes\'us Biel y Paco Ramos. Sin el ambiente de trabajo y camarader\'ia presente en el grupo, sencillamente esta tesis no hubiera llegado a buen puerto.


Siento una especial gratitud tanto a nivel profesional como personal hacia Baruch Meerson. A\'un me sorprenden su compromiso y dedicaci\'on, sus sinceros consejos, as\'i como su cari\~no y cercan\'ia, los cuales me ayudaron a creer en esta tesis y est\'an m\'as all\'a de todo elogio. Tampoco podr\'e olvidar el excelente recibimiento que me brindaron \'el y su esposa en esa ciudad maravillosa que es Jerusal\'en.

Durante estos a\~nos he tenido dos buenos colaboradores en Thorsten P\"oschel y Thomas Schwager, a los que les agradezco todo su inter\'es y la doblemente buena acogida dispensada en Berl\'in.

Qu\'e importantes han sido los amigos, siempre presentes, de los que hay poco que decir y mucho que agradecer. En este periplo he tenido la gran suerte de conocer a Juan Antonio, igualmente miembro del grupo. Con \'el he compartido innumerables charlas, preocupaciones, confidencias, confianza, amistad. Gracias. A mis ya viejos amigos: Fernando, que tambi\'en sabe lo que es hacer una tesis luchando d\'ia a d\'ia a tocapenoles, le debo su experiencia y su apoyo en momentos dif\'iciles; a Miguel, para m\'i m\'as que un amigo, por la ilusi\'on y el tiempo que juntos invertimos en tantos proyectos; a Jes\'us, por su ejemplar honradez y fidelidad, y al resto de los miembros del equipo. 

A mis padres, que lo han dado todo por m\'i. A Gabi, Holger y Christoph, por su continuo inter\'es y cari\~no.

A Cora, porque a pesar de haber demorado la redacci\'on de este trabajo me ha alegrado la vida. Y finalmente a Linda, mi esposa y mi gu\'ia, a quien le dedico esta tesis. %: ha estado a mi lado, ha disfrutado y sufrido conmigo. %, mi faro, mi gu\'ia. 
Gracias por todo, lo decible y lo indecible.

\vspace{2cm}
\begin{flushright}
Granada, a 17 de Septiembre de 2006.
\end{flushright}


